3D-UCaps: 3D Capsules Unet for Volumetric Image Segmentation

Medical image segmentation has been so far achieving promising results with Convolutional Neural Networks (CNNs). However, it is arguable that in traditional CNNs, its pooling layer tends to discard important information such as positions. Moreover, CNNs are sensitive to rotation and affine transformation. Capsule network is a data-efficient network design proposed to overcome such limitations by replacing pooling layers with dynamic routing and convolutional strides, which aims to preserve the part-whole relationships. Capsule network has shown a great performance in image recognition and natural language processing, but applications for medical image segmentation, particularly volumetric image segmentation, has been limited. In this work, we propose 3D-UCaps, a 3D voxel-based Capsule network for medical volumetric image segmentation. We build the concept of capsules into a CNN by designing a network with two pathways: the first pathway is encoded by 3D Capsule blocks, whereas the second pathway is decoded by 3D CNNs blocks. 3D-UCaps, therefore inherits the merits from both Capsule network to preserve the spatial relationship and CNNs to learn visual representation. We conducted experiments on various datasets to demonstrate the robustness of 3D-UCaps including iSeg-2017, LUNA16, Hippocampus, and Cardiac, where our method outperforms previous Capsule networks and 3D-Unets.

==> MICCAI2021 SegCaps3D/submission/rebuttal.tex <==
We thank the reviewers for their feedback. We are glad to receive positive comments that value the contribution of our work. We clarify the key points and then address specific concerns individually.


## MAJOR CONCERNS

**KP1. Reproducibility and expandability**

We will release both source code and pre-trained models. Our code is implemented with Pytorch Lightning with MONAI framework for processing data, running sliding window inference and computing dice score with fixed seed. We hope that by having up-to-date frameworks, the community can reproduce our results and extend our method to other problems.

**KP2. Motion artifacts** 

Motion artifact is a complex problem with many partial solutions as given in Zaitsev et al., Motion artifacts in MRI: A complex problem with many partial solutions, Journal of Magnetic Resonance Imaging, 2015. In this work, we simplify the motion artifacts caused by patient movement during scanning by rotating 20\% number of slides with angle randomly chosen from  (-5, 5) degrees around x/y/z-axis. More realistic experiments with various k-space motion artifacts argumentation will be examined with TorchIO in our future study.

**KP3. "Performance of 3D SegCaps on the LUNA16, Hippocampus, cardiac datasets"**

Our best trial for 3D SegCaps produced result no better than [24], and so we have shifted the focus to our proposed method. The possible answer for this problem can be seen in the third concern of Reviewer 1. As per request, we will provide additional segmentation performance of 3D SegCaps to get a full comparison.


## INDIVIDUAL CONCERNS

**Reviewer 1**

1. Reproducibility: Please refer KP1.

2. Demonstration: Qualitative results will be made as a supplementary and will be added to the code release.

3. The empirical finding, i.e., the expanding path has negligible effects"
Further investigation is needed to understand the effects of capsules in the expanding path. In our hypothesis, routing algorithm works based on routing-by-agreement between part to whole relationship, however the relationship between whole to part is one-to-many, and it is ambiguous to find the agreement between whole to active corresponding parts. 

4. Multi-class segmentation: We have conducted the experimental results on multi-class segmentation with 3D UCaps as given in Tables 1, 2, 3  on iSeg dataset with 3 classes i.e. WT, GM, CSF.


**Reviewer 3**

1. "3D SkipDense instead of 3D U-Net which is more popular in the literature when considering rotation invariance and motion artifacts?" 

We are motivated by the iSeg2017 challenge [26] in which all participating methods performed poorly on the testing subjects acquired with motion artifacts and unusual scan poses. We choose to report 3D SkipDense as this method is proposed in 2019 and has the state-of-the-art performance. Their code and pretrained model are also publicly available. 

2. "When the the rotation variance is created for the testing dataset, was this random? Also, what would happen if the rotation was in x-axis or y-axis or both x- and y- axes or all axes? How is the performance affected if those rotations happen?"

We trained our network with provided data in the dataset without any rotation data augmentation. During testing, we choose an axis to rotate the volume, and apply the rotation with angle values fixed to 5, 10, 15, .., 90 degrees. In our experiment, the performance tends to drop slightly when the rotation angles increases. We also found that rotating about a single axis or all axes does not have significant performance difference, which explains the capability to handle rotation invariance in a capsule network.









==> MICCAI2021 SegCaps3D/submission/tmp.tex <==
%This preservation capability has been proven by 'reverse engineering" i.e., reconstructing the input from the output capsule vectors. 
%Due to robustness to the rotation, affine transformations, intrinsic spatial preservation, Capsule network can effectively solve the limitations of CNNs and achieve the expected performance with less training data, which are very important for medical image analysis. 




%Particularly, a capsule is a group of neurons that represent different properties of the same entity such as pose, deformation, texture, etc. When these properties of the entity change in the input, their neuron activation will change accordingly, and the network can still recognize the object successfully while preserving important information of the object and its parts. These strengths of capsule networks can be very beneficial in the context of medical image segmentation where the data is limited, and there are large variations among training samples. 

% In this work, we propose a 3D voxel-based capsule network for a variety of medical image segmentation tasks: tissue segmentation, organ segmentation, and tumor segmentation.
% By observing that a capsule network can effectively encode the spatial relationship from parts to object but not the opposite, we propose a hybrid encoder-decoder neural network for segmentation: we use capsules in the encoder to learn rich object representations in low resolutions and then use transposed convolutions with skip connections to output high-resolution segmentation results. 
% We show that our network is easier to train, having better results compared to previous 2D capsule networks on the same task, and having fewer parameters than traditional neural networks.



\begin{itemize}[leftmargin=*]
    \item Binary segmentation: most up-to-date CapsNet for MIS \cite{lalonde2018capsules,lalonde2021capsules,he2020automatic} is implemented with binary segmentation task only while many of medical tasks require multi-classes. Lately, \cite{survarachakan2020capsule} shows difficulty when extending binary Segcap \cite{lalonde2018capsules} to an arbitrary number of classes;
    \item Lack of temporal information: all CapsNet for either image classification or image segmentation has been designed as a 2D network for 2D images only while most medical data is more than 2-dimensions i.e., MRI, X-ray, PET. To apply such CapsNet to medical data, each volumetric slide has been processed independently. Thus, temporal information between volumetric slides can not be taken into account.
    \item CapsNet for MIS has followed by Unet-like architecture and replaced pooling layers  with dynamic routing mechanism. In such networks, deconvolutional Capsules have been introduced in the decoder pathway. However,  \hl{need to discuss}
\end{itemize}



While we agree with SegCaps \cite{lalonde2018capsules,lalonde2021capsules,he2020automatic} that convolutional Capsules presents the part-whole relationship,
To prove this argument, we will compare our proposed 3D-UCaps in two cases when the decoder is designed by 3D CNNs blocks and 3D Capsules blocks.




%Many modalities, e.g., X-ray, CT, MRI, etc. have been used for acquiring medical images. 
% In the era of deep learning, convolutional neural networks (CNNs) have been applied for medical image segmentation, showing promising results on a variety of data modalities (X-ray, CT, MRI, etc.) and data domains (organs, tumors, etc.). 


% Among the image modalities, medical image segmentation with 3D data, e.g., MRI, has received great attention. 
% Building a neural network to segment an MRI image is challenging in that MRI data can be limited. 


% A potential way to alleviate such problem is to preserve more information from the input during learning. 
% Capsule networks~\cite{} allow part-whole relationship in the data, which can be applied for medical image segmentation. 
% LaLonde and Bagci~\cite{lalonde2018capsules} attempted to use a capsule network to build an encoder-decoder for object segmentation, which is shown to have comparable segmentation performance to traditional methods for medical image segmentation. 
% A limitation of their method is that they treat MRI as slices of 2D images, which disregards temporal information in the learning. 


% In this work, we propose to lift the capsule network to the 3D domain. We propose to use capsules to encode the spatial relationship from parts to whole objects, and use a convolutional decoder to output high-resolution segmentation results. 
% We show that our 3D capsule network can outperform SegCaps~\cite{}, and work as efficient as convolutional neural networks in the medical image segmentation task. 





%--- Introduce Capsule Network and how it has been utilized in Medical Image Segmentation

%- Limitations of 2D Segcap: do not take temporal into consideration. Segcap performs well on most of medical datasets
%- Contributions
%+ Network designs:
%    + Encoder - Capsule
%    + Decoder - Convolution 
%+ Performance



\begin{table}[t]
    \caption{The details of our neural network. Refer to Figure~\ref{fig:rinet} for an illustration of the network architecture, and Algorithm~\ref{alg:conv} for steps in \ourconv operator. Here, K is the number of categories.}
    \label{tab:network}
    \centering
    \begin{tabular}{l | c} 
        \noalign{\smallskip}\hline\noalign{\smallskip}
        Module & Output shape\\
        \noalign{\smallskip}\hline\noalign{\smallskip}
        \textbf{\ourconv} & \\
        Input tensor  & in\_planes $\times$ in\_points \\
        RIConv++ operator & out\_planes $\times$ out\_points \\
        BatchNorm & out\_planes $\times$ out\_points \\
        ReLU &  out\_planes $\times$ out\_points \\
        \\
        \textbf{Classification / Retrieval} & \\
        Input tensor & $3 \times 1024$ \\
        \ourconv & $128 \times 256$ \\
        \ourconv & $256 \times 128$ \\
        \ourconv & $512 \times 64$\\
        Fully connected & $256 \times 1$ \\
        Fully connected & $128 \times 1$ \\ 
        Softmax & $K \times 1$ \\
        \\
        \textbf{Segmentation} & \\
        Input tensor & $3 \times 2048$ \\
        \ourconv & $128 \times 512$ \\
        \ourconv & $256 \times 128$ \\
        \ourconv & $512 \times 64$
        \vspace{0.05in}\\
        \ourconv & $256 \times 128$ \\
        Skip connection & $512 \times 128$ \\
        MLP & $256 \times 128$ \\
        \ourconv & $128 \times 512$ \\
        Skip connection & $256 \times 512$ \\
        MLP & $128 \times 512$ \\
        \ourconv & $K \times 2048$ \\
        \noalign{\smallskip}\hline\noalign{\smallskip}
    \end{tabular}
\end{table}




% \subsection{Capsule-based Medical Image Segmentation}


% TODO: move to another location 

% We used infant brain MRI dataset from iSeg 2017 challenge \cite{wang2019benchmark} as a main dataset to compare the performance and robustness of our method against other approaches. It has some desired properties when compared to LUNA16 dataset \cite{setio2017validation} that was used in SegCaps \cite{lalonde2018capsules} work.
%(1) The ground-truth annotations were manually segmentation under the guidance of an experienced neuroradiologist while segmentation masks of LUNA16 were created by an automated algorithm \cite{van2009automatic}.
%(2) This is a multi-class segmentation task with multi-modalities while they provided T1w and T2w images for each subject and we have to segment the infant brain into four regions: cerebrospinal fluid (CSF), white matter (WM), gray matter (GM), and background that have more complex shape than lung segmentation.
%(3) They have reported in \cite{wang2019benchmark} that all previous methods performed badly on subjects with motion and unusual scan pose. We will resemble this transformation and show that our method is more robust thanks to the viewpoint equivariance property of capsule encoder. Besides that, we also experiment on LUNA16 dataset, cardiac and hippocampus dataset from the Medical Segmentation Decathlon \cite{simpson2019large} to compare with other capsule-based network works \cite{lalonde2018capsules,survarachakan2020capsule}. The details of each dataset are:




\noindent \textbf{iSeg:} The iSeg17 dataset \cite{wang2019benchmark} consists of 10 subjects with ground-truth labels for training and 13 subjects without ground-truth labels for testing. Each subject includes T1 and T2 images with size of $144 \times 192 \times 256$, and image resolution of $1 \times 1 \times 1$  $\text{mm}^3$. In iSeg, there are three classes:  white matter (WM), gray matter (GM), and cerebrospinal fluid (CSF). We follow the experiment setup by 3D-SkipDenseSeg \cite{bui2019skip} to conduct the report on this dataset where 9 subjects are use for training and 1 subject (subject \#9) is for testing.


% In iSeg, there are three classes:  white matter (WM), gray matter (GM), and cerebrospinal fluid (CSF)

% \noindent \textbf{Pancreas:}Pancreas~\cite{pancreas} contains 82 abdominal contrast enhanced 3D CT scans. The CT scans have resolutions of $512 \times 512 \times xxx$    pixels with varying pixel sizes and slice thickness between 1.5--2.5 mm.

\noindent \textbf{Luna:} A LUNA \cite{luna} contains 888 CT scans, each scan with size of $512 \times 512 \times xxx$. Different from most of the medical datasets which were annotated by clinical experts (radiologists). Ground-truth annotations in LUNA were created by an automated algorithm \cite{van2009automatic}. We follow similar experiment setup in SegCaps~\cite{lalonde2018capsules} to conduct the results on LUNA. We randomly split the dataset into four training/testing folds for performing k-fold cross-validation. \hl{Furthermore, we removed 10 of the 888 CT scans due to exceedingly poor annotations}.

\noindent \textbf{Cardiac:} is a mono-modal MRI dataset which contains 20 training images and 10 testing images. To conduct the experimental results on Cardiac, we randomly split the training set into four training/testing folds for performing k-fold cross-validation.  

\noindent \textbf{Hippocampus:} is a larger-scale mono-modal MRI dataset. It  consists of 260 training and 130 testing samples. We also use 4-fold cross validation on training set to conduct the experiments results.


% We perform experiments on various medical image segmentation datasets to validate our method. 
% Specifically, we test with iSeg, Luna16, Hippocampus, and Atrium.
% iSeg is a MRI dataset of infant brains that requires to be segmented into white matter (WM), gray matter (GM), and cerebrospinal fluid (CSF).
% Luna16 contains chest CT scans for analyzing lung nodules. 
% Hippocampus is for evaluating segmentation masks for brain MRIs. 
% Atrium contains 30 MRI images for left atrium segmentation. 

==> MICCAI2021 SegCaps3D/submission/tmp/Rebuttal_V1.tex <==
% Please put your rebuttal here. Max 4000 characters. 

We thank the reviewers for their feedback. We are glad to receive positive comments that value the contribution of our work. We clarify the key points and then address specific concerns individually.

## MAJOR CONCERNS

**KP1. Reproducibility: we will release both code and pre-trained models, as promised. 

**KP2. "Results for 3D SegCaps for the LUNA16, Hippocampus, cardiac datasets"

SegCaps3D is an improvement of SegCaps2D by replacing 2D conv with 3D conv. As shown in [24], SegCaps2D must be trained on Stochastic Gradient Descent (SGD). If not, it is not converged. Employing the same configuration, SegCaps3D is trained with SGD. Compare to other datasets, iSeg is the smallest dataset and it is multi-class segmentation. Thus, we conduct the performance of SegCaps3D on iSeg. As per request, we will provide additional segmentation performance of SegCaps3D on other datasets in the supplementary material and in the code release. 

% Where is the connection here?
% Compare to other datasets, iSeg is the smallest dataset and it is multi-class segmentation. Thus, we conduct the performance of SegCaps3D on iSeg. 

%As per request, we will provide additional segmentation performance of SegCaps3D on other datasets in the supplementary material and in the code release. 

%3D SegCaps is an improvement of 2D SegCaps by replacing 2D convolution with 3D convolution. As shown in [24], 2D SegCaps provided poor results on other datasets, which could be due to randomness in sampling order or weight initialization. We also found out that 2D/3D SegCaps must be trained on Stochastic Gradient Descent (SGD), else the training does not converge. Because of this additional high computational cost of capsule network due to iterative routing algorithm, we only train 3D SegCaps for the smallest dataset iSeg2017 which has 9 samples.

**KP3. Motion artifacts: Motion artifact is a complex problem with many partial solutions as given in Zaitsev et al., "Motion artifacts in MRI: A complex problem with many partial solutions. J Magn Reson Imaging. In this work, the motion artifacts is created by randomly rotating 20\% number of slides. We believe that our work provides the first investigating the influence of motion artifact to capsule-based deep networks. Capsule-based deep network with various k-space motion artifacts argumentation will be examined with torchIO in our coming study.

%We believe that our work provides the first investigation of the influence of motion artifacts to capsule-based deep networks. Capsule-based deep network with various k-space motion artifacts argumentation will be examined with TorchIO, an efficient library for processing medical images in our future study.

## INDIVIDUAL CONCERNS

**Reviewer 1**
1. Reproducibility: Please refer KP1.
2. Demonstration: Qualitative results will be made as a supplementary and will be added to the code release.

3. Empirical finding:
In our hypothesis, the current complexity and high computation cost hinders the decoding capsules from being well optimized. 
TODO: Please cite the the paper ...

4. Multi-class segmentation:
 We have conducted the experimental results on multi-class segmentation with 3D SegCaps as given in Tables 1, 2, 3  on iSeg dataset with 3 classes i.e. WT, GM, CSF.

%the only challenge I can find from this keyword is "https://www.aicrowd.com/challenges/hecktor" however it is still a binary segmentation challenge. I think use capsule network for multi-label segmentation task can be a great idea and actually we can consider BraTS as this type of challenge. 
**Reviewer 3**
1. Results for 3D SegCaps for the LUNA16, Hippocampus, cardiac datasets: Please refer KP2. 

2. Compare to 3D SkipDense instead of 3D U-Net:  3D SkipDense [3] was proposed in 2019 and it is an improvement of 3D U-Net [5]. In our work, we have make comparison on both 3D SkipDense [3] and 3D U-Net [5] as given in Table 1. Furthermore, [3] is one of the state-of-the-art method on iSeg dataset.

3. Motion artifacts: Please refer KP3.
4. Was rotation variance is created randomly?: Yes it was
TODO: explain more details about rotation experiment, 



"When the the rotation variance is created for the testing dataset, was this random? Also, what would happen if the rotation was in x-axis or y-axis or both x- and y- axes or all axes? How is the performance affected if those rotations happen?"
TODO: explain more detailed about rotation experiment, 

#Draft version

We thank the reviewers for their feedback. We are glad to receive positive comments that value the contribution of our work. In summary, we group reviewer concern into three main problems.

The first one is the effectiveness of our architecture. Reviewer 3 ask why we do not provide any results for 3D SegCaps for other datasets beside iSeg2017 and the reason it's we can only train 3D SegCaps successfully if we set the training batch size to 1 or it will produce very low result which have been shown in [24]. Because of this plus high computational cost of capsule network due to iterative routing algorithm, we only train 3D SegCaps for the smallest dataset iSeg2017 which has 9 samples. On the other hand, our network with convolutional decoder do not suffer from this problem and for example, we can train with batch size 32 for patch size (32, 32, 32) on 32GB V100 GPU. Our hypothesis for this empirical finding, which also address reviewer 1 concern on our expanding path, is routing algorithm working based on routing-by-agreement between part to whole relationship, however the relationship between whole to part is one-to-many, we do not find the agreement between whole to active corresponding parts. Then we think the job of expanding path is learning the latent representation of the "whole" capsules from contracting path and replicating the knowledge spatially, which is the purpose of convolutational layers
#####Then we think the job of expanding path is learning the latent representation of the "whole" capsules from contracting path and replicating the knowledge spatially, which is the purpose of convolutational layers

The second one is the experimental choices in our work. Our motivation for robustness experiment come from the reporting of iSeg2017 challenge [26] in which all methods consistently performed badly on the testing subjects acquired with motion artifacts and unusual scan pose. Among participant methods, 3D SkipDense not only stand out because of its performance but they also publish their code and pretrained model on github. Then we can easily check the result and perform our robustness experiment on their model. About the rotation invariance experiment, the result was collected by rotating the testing subject around z-axis with different angles in this order: 0, 5, 15, 30, 45, 60, 75, 90 then there was no random as reviewer 3 concerned. The same results was collected if we rotate testing subject around x-axis, y-axis or all axis as reviewer 3 suggested but we did not have enough space to put these results into the paper. Then we will show them below

| Rotate axis | Model           | 0     | 5     | 15    | 30    | 45    | 60    | 75    | 90    |
|-------------|-----------------|-------|-------|-------|-------|-------|-------|-------|-------|
| x           | 3D-SkipDense    | 92.51 | 89.86 | 72.98 | 74.25 | 86.70 | 85.64 | 84.89 | 85.96 |
|             | 3D-UCaps (ours) | 92.17 | 89.53 | 89.09 | 87.92 | 86.70 | 85.64 | 84.89 | 85.96 |
| y           | 3D-SkipDense    | 92.51 | 89.36 | 69.51 | 76.06 | 74.25 | 74.25 | 74.25 | 74.25 |
|             | 3D-UCaps (ours) | 92.17 | 89.41 | 89.01 | 88.22 | 87.46 | 86.86 | 86.47 | 88.01 |
| all         | 3D-SkipDense    | 92.51 | 89.67 | 82.97 | 83.02 | 74.25 | 74.25 | 74.25 | 74.25 |
|             | 3D-UCaps (ours) | 92.17 | 89.67 | 82.97 | 83.02 | 74.25 | 74.25 | 74.25 | 74.25 |

The last one is the reproducibility and expandability of our work. We have refactored our code so it use MONAI framework for processing data, running sliding window inference and computing dice score with fixed seed. We also follow Pytorch Lightning framework to organize our code effectively. We hope that by using these popular and up-to-date frameworks, anyone in the community can reproduce our results correctly and extend our method easily to other problems as reviewer 1 suggested.

%TODO: explain more detailed about rotation experiment, 
%The result was collected by rotating the testing subject around z-axis with different angles in this order: 0, 5, 15, 30, 45, 60, 75, 90 then there was no random here. The same results was collected if we rotate testing subject around x-axis, y-axis or all axis as you can see in the table below

%| Rotate axis | Model           | 0     | 5     | 15    | 30    | 45    | 60    | 75    | 90    |
%|-------------|-----------------|-------|-------|-------|-------|-------|-------|-------|-------|
%| x           | 3D-SkipDense    | 92.51 | 89.38 | 88.99 | 88.16 | 87.16 | 86.27 | 85.59 |  |
%|             | 3D-UCaps (ours) | 92.17 | 89.53 | 89.09 | 87.92 | 86.70 | 85.64 | 84.89 | 85.96 |
%| y           | 3D-SkipDense    | 92.51 | 89.46 | 89.17 | 88.67 | 88.06 | 87.53 | 87.10 | 89.13 |
%|             | 3D-UCaps (ours) | 92.17 | 89.41 | 89.01 | 88.22 | 87.46 | 86.86 | 86.47 | 88.01 |
%| all         | 3D-SkipDense    | 92.51 | 87.70 | 86.90 | 85.33 | 83.84 | 83.00 | 82.47 | 85.28 |
%|             | 3D-UCaps (ours) | 92.17 | 88.17 | 87.26 | 85.09 | 83.40 | 82.05 | 81.12 | 83.64 |

| Rotate axis | Model           | 0     | 5     | 15    | 30    | 45    | 60    | 75    | 90    |
|-------------|-----------------|-------|-------|-------|-------|-------|-------|-------|-------|
| x           | 3D-SkipDense    | 92.60 | 89.38 | 88.99 | 88.16 | 87.16 | 86.27 | 85.59 | 87.04 |
|             | 3D-UNet         | 92.48 | 89.61 | 89.16 | 87.98 | 86.74 | 85.63 | 84.97 | 86.41 |
|             | 3D-UCaps (ours) | 92.54 | 89.79 | 89.23 | 88.00 | 86.71 | 85.65 | 84.97 | 86.31 |
| y           | 3D-SkipDense    | 92.60 | 89.46 | 89.17 | 88.67 | 88.06 | 87.53 | 87.10 | 89.13 |
|             | 3D-UNet         | 92.48 | 89.61 | 89.16 | 88.21 | 87.30 | 86.69 | 86.19 | 87.87 |
|             | 3D-UCaps (ours) | 92.54 | 89.82 | 89.40 | 88.53 | 87.79 | 87.19 | 86.73 | 88.49 |
| all         | 3D-SkipDense    | 92.60 | 87.70 | 86.90 | 85.33 | 83.84 | 83.00 | 82.47 | 85.28 |
|             | 3D-UNet         | 92.48 | 88.29 | 87.14 | 84.94 | 83.22 | 82.06 | 81.13 | 83.81 |
|             | 3D-UCaps (ours) | 92.54 | 88.46 | 87.27 | 85.13 | 83.58 | 82.48 | 81.64 | 84.27 |

==> MICCAI2021 SegCaps3D/submission/tmp/rebuttal_Tan.tex <==
#Draft version

We thank the reviewers for their feedback. We are glad to receive positive comments that value the contribution of our work. In summary, we group reviewer concern into three main problems.

The first one is the effectiveness of our architecture. Reviewer 3 ask why we do not provide any results for 3D SegCaps for other datasets beside iSeg2017 and the reason it's we can only train 3D SegCaps successfully if we set the training batch size to 1 or it will produce very low result which have been shown in [24]. Because of this plus high computational cost of capsule network due to iterative routing algorithm, we only train 3D SegCaps for the smallest dataset iSeg2017 which has 9 samples. On the other hand, our network with convolutional decoder do not suffer from this problem and for example, we can train with batch size 32 for patch size (32, 32, 32) on 32GB V100 GPU. Our hypothesis for this empirical finding, which also address reviewer 1 concern on our expanding path, is routing algorithm working based on routing-by-agreement between part to whole relationship, however the relationship between whole to part is one-to-many, we do not find the agreement between whole to active corresponding parts. Then we think the job of expanding path is learning the latent representation of the "whole" capsules from contracting path and replicating the knowledge spatially, which is the purpose of convolutational layers

The second one is the experimental choices in our work. Our motivation for robustness experiment come from the reporting of iSeg2017 challenge [26] in which all methods consistently performed badly on the testing subjects acquired with motion artifacts and unusual scan pose. Among participant methods, 3D SkipDense not only stand out because of its performance but they also publish their code and pretrained model on github. Then we can easily check the result and perform our robustness experiment on their model. About the rotation invariance experiment, the result was collected by rotating the testing subject around z-axis with different angles in this order: 0, 5, 15, 30, 45, 60, 75, 90 then there was no random as reviewer 3 concerned. The same results was collected if we rotate testing subject around x-axis, y-axis or all axis as reviewer 3 suggested but we did not have enough space to put these results into the paper. Then we will show them below

| Rotate axis | Model           | 0     | 5     | 15    | 30    | 45    | 60    | 75    | 90    |
|-------------|-----------------|-------|-------|-------|-------|-------|-------|-------|-------|
| x           | 3D-SkipDense    | 92.51 | 89.86 | 72.98 | 74.25 | 86.70 | 85.64 | 84.89 | 85.96 |
|             | 3D-UCaps (ours) | 92.17 | 89.53 | 89.09 | 87.92 | 86.70 | 85.64 | 84.89 | 85.96 |
| y           | 3D-SkipDense    | 92.51 | 89.36 | 69.51 | 76.06 | 74.25 | 74.25 | 74.25 | 74.25 |
|             | 3D-UCaps (ours) | 92.17 | 89.41 | 89.01 | 88.22 | 87.46 | 86.86 | 86.47 | 88.01 |
| all         | 3D-SkipDense    | 92.51 | 87.70 | 86.90 | 85.33 | 83.84 | 83.00 | 82.47 | 85.28 |
|             | 3D-UCaps (ours) | 92.17 | 88.17 | 87.26 | 85.09 | 83.40 | 82.05 | 81.12 | 83.64 |

The last one is the reproducibility and expandability of our work. We have refactored our code so it use MONAI framework for processing data, running sliding window inference and computing dice score with fixed seed. We also follow Pytorch Lightning framework to organize our code effectively. We hope that by using these popular and up-to-date frameworks, anyone in the community can reproduce our results correctly and extend our method easily to other problems as reviewer 1 suggested. 

==> submission/rebuttal.tex <==
We thank the reviewers for their feedback. We are glad to receive positive comments that value the contribution of our work. We clarify the key points and then address specific concerns individually.


## MAJOR CONCERNS

**KP1. Reproducibility and expandability**

We will release both source code and pre-trained models. Our code is implemented with Pytorch Lightning with MONAI framework for processing data, running sliding window inference and computing dice score with fixed seed. We hope that by having up-to-date frameworks, the community can reproduce our results and extend our method to other problems.

**KP2. Motion artifacts** 

Motion artifact is a complex problem with many partial solutions as given in Zaitsev et al., Motion artifacts in MRI: A complex problem with many partial solutions, Journal of Magnetic Resonance Imaging, 2015. In this work, we simplify the motion artifacts caused by patient movement during scanning by rotating 20\% number of slides with angle randomly chosen from  (-5, 5) degrees around x/y/z-axis. More realistic experiments with various k-space motion artifacts argumentation will be examined with TorchIO in our future study.

**KP3. "Performance of 3D SegCaps on the LUNA16, Hippocampus, cardiac datasets"**

Our best trial for 3D SegCaps produced result no better than [24], and so we have shifted the focus to our proposed method. The possible answer for this problem can be seen in the third concern of Reviewer 1. As per request, we will provide additional segmentation performance of 3D SegCaps to get a full comparison.


## INDIVIDUAL CONCERNS

**Reviewer 1**

1. Reproducibility: Please refer KP1.

2. Demonstration: Qualitative results will be made as a supplementary and will be added to the code release.

3. The empirical finding, i.e., the expanding path has negligible effects"
Further investigation is needed to understand the effects of capsules in the expanding path. In our hypothesis, routing algorithm works based on routing-by-agreement between part to whole relationship, however the relationship between whole to part is one-to-many, and it is ambiguous to find the agreement between whole to active corresponding parts. 

4. Multi-class segmentation: We have conducted the experimental results on multi-class segmentation with 3D UCaps as given in Tables 1, 2, 3  on iSeg dataset with 3 classes i.e. WT, GM, CSF.


**Reviewer 3**

1. "3D SkipDense instead of 3D U-Net which is more popular in the literature when considering rotation invariance and motion artifacts?" 

We are motivated by the iSeg2017 challenge [26] in which all participating methods performed poorly on the testing subjects acquired with motion artifacts and unusual scan poses. We choose to report 3D SkipDense as this method is proposed in 2019 and has the state-of-the-art performance. Their code and pretrained model are also publicly available. 

2. "When the the rotation variance is created for the testing dataset, was this random? Also, what would happen if the rotation was in x-axis or y-axis or both x- and y- axes or all axes? How is the performance affected if those rotations happen?"

We trained our network with provided data in the dataset without any rotation data augmentation. During testing, we choose an axis to rotate the volume, and apply the rotation with angle values fixed to 5, 10, 15, .., 90 degrees. In our experiment, the performance tends to drop slightly when the rotation angles increases. We also found that rotating about a single axis or all axes does not have significant performance difference, which explains the capability to handle rotation invariance in a capsule network.









==> submission/tmp.tex <==
%This preservation capability has been proven by 'reverse engineering" i.e., reconstructing the input from the output capsule vectors. 
%Due to robustness to the rotation, affine transformations, intrinsic spatial preservation, Capsule network can effectively solve the limitations of CNNs and achieve the expected performance with less training data, which are very important for medical image analysis. 




%Particularly, a capsule is a group of neurons that represent different properties of the same entity such as pose, deformation, texture, etc. When these properties of the entity change in the input, their neuron activation will change accordingly, and the network can still recognize the object successfully while preserving important information of the object and its parts. These strengths of capsule networks can be very beneficial in the context of medical image segmentation where the data is limited, and there are large variations among training samples. 

% In this work, we propose a 3D voxel-based capsule network for a variety of medical image segmentation tasks: tissue segmentation, organ segmentation, and tumor segmentation.
% By observing that a capsule network can effectively encode the spatial relationship from parts to object but not the opposite, we propose a hybrid encoder-decoder neural network for segmentation: we use capsules in the encoder to learn rich object representations in low resolutions and then use transposed convolutions with skip connections to output high-resolution segmentation results. 
% We show that our network is easier to train, having better results compared to previous 2D capsule networks on the same task, and having fewer parameters than traditional neural networks.



\begin{itemize}[leftmargin=*]
    \item Binary segmentation: most up-to-date CapsNet for MIS \cite{lalonde2018capsules,lalonde2021capsules,he2020automatic} is implemented with binary segmentation task only while many of medical tasks require multi-classes. Lately, \cite{survarachakan2020capsule} shows difficulty when extending binary Segcap \cite{lalonde2018capsules} to an arbitrary number of classes;
    \item Lack of temporal information: all CapsNet for either image classification or image segmentation has been designed as a 2D network for 2D images only while most medical data is more than 2-dimensions i.e., MRI, X-ray, PET. To apply such CapsNet to medical data, each volumetric slide has been processed independently. Thus, temporal information between volumetric slides can not be taken into account.
    \item CapsNet for MIS has followed by Unet-like architecture and replaced pooling layers  with dynamic routing mechanism. In such networks, deconvolutional Capsules have been introduced in the decoder pathway. However,  \hl{need to discuss}
\end{itemize}



While we agree with SegCaps \cite{lalonde2018capsules,lalonde2021capsules,he2020automatic} that convolutional Capsules presents the part-whole relationship,
To prove this argument, we will compare our proposed 3D-UCaps in two cases when the decoder is designed by 3D CNNs blocks and 3D Capsules blocks.




%Many modalities, e.g., X-ray, CT, MRI, etc. have been used for acquiring medical images. 
% In the era of deep learning, convolutional neural networks (CNNs) have been applied for medical image segmentation, showing promising results on a variety of data modalities (X-ray, CT, MRI, etc.) and data domains (organs, tumors, etc.). 


% Among the image modalities, medical image segmentation with 3D data, e.g., MRI, has received great attention. 
% Building a neural network to segment an MRI image is challenging in that MRI data can be limited. 


% A potential way to alleviate such problem is to preserve more information from the input during learning. 
% Capsule networks~\cite{} allow part-whole relationship in the data, which can be applied for medical image segmentation. 
% LaLonde and Bagci~\cite{lalonde2018capsules} attempted to use a capsule network to build an encoder-decoder for object segmentation, which is shown to have comparable segmentation performance to traditional methods for medical image segmentation. 
% A limitation of their method is that they treat MRI as slices of 2D images, which disregards temporal information in the learning. 


% In this work, we propose to lift the capsule network to the 3D domain. We propose to use capsules to encode the spatial relationship from parts to whole objects, and use a convolutional decoder to output high-resolution segmentation results. 
% We show that our 3D capsule network can outperform SegCaps~\cite{}, and work as efficient as convolutional neural networks in the medical image segmentation task. 





%--- Introduce Capsule Network and how it has been utilized in Medical Image Segmentation

%- Limitations of 2D Segcap: do not take temporal into consideration. Segcap performs well on most of medical datasets
%- Contributions
%+ Network designs:
%    + Encoder - Capsule
%    + Decoder - Convolution 
%+ Performance



\begin{table}[t]
    \caption{The details of our neural network. Refer to Figure~\ref{fig:rinet} for an illustration of the network architecture, and Algorithm~\ref{alg:conv} for steps in \ourconv operator. Here, K is the number of categories.}
    \label{tab:network}
    \centering
    \begin{tabular}{l | c} 
        \noalign{\smallskip}\hline\noalign{\smallskip}
        Module & Output shape\\
        \noalign{\smallskip}\hline\noalign{\smallskip}
        \textbf{\ourconv} & \\
        Input tensor  & in\_planes $\times$ in\_points \\
        RIConv++ operator & out\_planes $\times$ out\_points \\
        BatchNorm & out\_planes $\times$ out\_points \\
        ReLU &  out\_planes $\times$ out\_points \\
        \\
        \textbf{Classification / Retrieval} & \\
        Input tensor & $3 \times 1024$ \\
        \ourconv & $128 \times 256$ \\
        \ourconv & $256 \times 128$ \\
        \ourconv & $512 \times 64$\\
        Fully connected & $256 \times 1$ \\
        Fully connected & $128 \times 1$ \\ 
        Softmax & $K \times 1$ \\
        \\
        \textbf{Segmentation} & \\
        Input tensor & $3 \times 2048$ \\
        \ourconv & $128 \times 512$ \\
        \ourconv & $256 \times 128$ \\
        \ourconv & $512 \times 64$
        \vspace{0.05in}\\
        \ourconv & $256 \times 128$ \\
        Skip connection & $512 \times 128$ \\
        MLP & $256 \times 128$ \\
        \ourconv & $128 \times 512$ \\
        Skip connection & $256 \times 512$ \\
        MLP & $128 \times 512$ \\
        \ourconv & $K \times 2048$ \\
        \noalign{\smallskip}\hline\noalign{\smallskip}
    \end{tabular}
\end{table}




% \subsection{Capsule-based Medical Image Segmentation}


% TODO: move to another location 

% We used infant brain MRI dataset from iSeg 2017 challenge \cite{wang2019benchmark} as a main dataset to compare the performance and robustness of our method against other approaches. It has some desired properties when compared to LUNA16 dataset \cite{setio2017validation} that was used in SegCaps \cite{lalonde2018capsules} work.
%(1) The ground-truth annotations were manually segmentation under the guidance of an experienced neuroradiologist while segmentation masks of LUNA16 were created by an automated algorithm \cite{van2009automatic}.
%(2) This is a multi-class segmentation task with multi-modalities while they provided T1w and T2w images for each subject and we have to segment the infant brain into four regions: cerebrospinal fluid (CSF), white matter (WM), gray matter (GM), and background that have more complex shape than lung segmentation.
%(3) They have reported in \cite{wang2019benchmark} that all previous methods performed badly on subjects with motion and unusual scan pose. We will resemble this transformation and show that our method is more robust thanks to the viewpoint equivariance property of capsule encoder. Besides that, we also experiment on LUNA16 dataset, cardiac and hippocampus dataset from the Medical Segmentation Decathlon \cite{simpson2019large} to compare with other capsule-based network works \cite{lalonde2018capsules,survarachakan2020capsule}. The details of each dataset are:




\noindent \textbf{iSeg:} The iSeg17 dataset \cite{wang2019benchmark} consists of 10 subjects with ground-truth labels for training and 13 subjects without ground-truth labels for testing. Each subject includes T1 and T2 images with size of $144 \times 192 \times 256$, and image resolution of $1 \times 1 \times 1$  $\text{mm}^3$. In iSeg, there are three classes:  white matter (WM), gray matter (GM), and cerebrospinal fluid (CSF). We follow the experiment setup by 3D-SkipDenseSeg \cite{bui2019skip} to conduct the report on this dataset where 9 subjects are use for training and 1 subject (subject \#9) is for testing.


% In iSeg, there are three classes:  white matter (WM), gray matter (GM), and cerebrospinal fluid (CSF)

% \noindent \textbf{Pancreas:}Pancreas~\cite{pancreas} contains 82 abdominal contrast enhanced 3D CT scans. The CT scans have resolutions of $512 \times 512 \times xxx$    pixels with varying pixel sizes and slice thickness between 1.5--2.5 mm.

\noindent \textbf{Luna:} A LUNA \cite{luna} contains 888 CT scans, each scan with size of $512 \times 512 \times xxx$. Different from most of the medical datasets which were annotated by clinical experts (radiologists). Ground-truth annotations in LUNA were created by an automated algorithm \cite{van2009automatic}. We follow similar experiment setup in SegCaps~\cite{lalonde2018capsules} to conduct the results on LUNA. We randomly split the dataset into four training/testing folds for performing k-fold cross-validation. \hl{Furthermore, we removed 10 of the 888 CT scans due to exceedingly poor annotations}.

\noindent \textbf{Cardiac:} is a mono-modal MRI dataset which contains 20 training images and 10 testing images. To conduct the experimental results on Cardiac, we randomly split the training set into four training/testing folds for performing k-fold cross-validation.  

\noindent \textbf{Hippocampus:} is a larger-scale mono-modal MRI dataset. It  consists of 260 training and 130 testing samples. We also use 4-fold cross validation on training set to conduct the experiments results.


% We perform experiments on various medical image segmentation datasets to validate our method. 
% Specifically, we test with iSeg, Luna16, Hippocampus, and Atrium.
% iSeg is a MRI dataset of infant brains that requires to be segmented into white matter (WM), gray matter (GM), and cerebrospinal fluid (CSF).
% Luna16 contains chest CT scans for analyzing lung nodules. 
% Hippocampus is for evaluating segmentation masks for brain MRIs. 
% Atrium contains 30 MRI images for left atrium segmentation. 

==> submission/tmp/Rebuttal_V1.tex <==
% Please put your rebuttal here. Max 4000 characters. 

We thank the reviewers for their feedback. We are glad to receive positive comments that value the contribution of our work. We clarify the key points and then address specific concerns individually.

## MAJOR CONCERNS

**KP1. Reproducibility: we will release both code and pre-trained models, as promised. 

**KP2. "Results for 3D SegCaps for the LUNA16, Hippocampus, cardiac datasets"

SegCaps3D is an improvement of SegCaps2D by replacing 2D conv with 3D conv. As shown in [24], SegCaps2D must be trained on Stochastic Gradient Descent (SGD). If not, it is not converged. Employing the same configuration, SegCaps3D is trained with SGD. Compare to other datasets, iSeg is the smallest dataset and it is multi-class segmentation. Thus, we conduct the performance of SegCaps3D on iSeg. As per request, we will provide additional segmentation performance of SegCaps3D on other datasets in the supplementary material and in the code release. 

% Where is the connection here?
% Compare to other datasets, iSeg is the smallest dataset and it is multi-class segmentation. Thus, we conduct the performance of SegCaps3D on iSeg. 

%As per request, we will provide additional segmentation performance of SegCaps3D on other datasets in the supplementary material and in the code release. 

%3D SegCaps is an improvement of 2D SegCaps by replacing 2D convolution with 3D convolution. As shown in [24], 2D SegCaps provided poor results on other datasets, which could be due to randomness in sampling order or weight initialization. We also found out that 2D/3D SegCaps must be trained on Stochastic Gradient Descent (SGD), else the training does not converge. Because of this additional high computational cost of capsule network due to iterative routing algorithm, we only train 3D SegCaps for the smallest dataset iSeg2017 which has 9 samples.

**KP3. Motion artifacts: Motion artifact is a complex problem with many partial solutions as given in Zaitsev et al., "Motion artifacts in MRI: A complex problem with many partial solutions. J Magn Reson Imaging. In this work, the motion artifacts is created by randomly rotating 20\% number of slides. We believe that our work provides the first investigating the influence of motion artifact to capsule-based deep networks. Capsule-based deep network with various k-space motion artifacts argumentation will be examined with torchIO in our coming study.

%We believe that our work provides the first investigation of the influence of motion artifacts to capsule-based deep networks. Capsule-based deep network with various k-space motion artifacts argumentation will be examined with TorchIO, an efficient library for processing medical images in our future study.

## INDIVIDUAL CONCERNS

**Reviewer 1**
1. Reproducibility: Please refer KP1.
2. Demonstration: Qualitative results will be made as a supplementary and will be added to the code release.

3. Empirical finding:
In our hypothesis, the current complexity and high computation cost hinders the decoding capsules from being well optimized. 
TODO: Please cite the the paper ...

4. Multi-class segmentation:
 We have conducted the experimental results on multi-class segmentation with 3D SegCaps as given in Tables 1, 2, 3  on iSeg dataset with 3 classes i.e. WT, GM, CSF.

%the only challenge I can find from this keyword is "https://www.aicrowd.com/challenges/hecktor" however it is still a binary segmentation challenge. I think use capsule network for multi-label segmentation task can be a great idea and actually we can consider BraTS as this type of challenge. 
**Reviewer 3**
1. Results for 3D SegCaps for the LUNA16, Hippocampus, cardiac datasets: Please refer KP2. 

2. Compare to 3D SkipDense instead of 3D U-Net:  3D SkipDense [3] was proposed in 2019 and it is an improvement of 3D U-Net [5]. In our work, we have make comparison on both 3D SkipDense [3] and 3D U-Net [5] as given in Table 1. Furthermore, [3] is one of the state-of-the-art method on iSeg dataset.

3. Motion artifacts: Please refer KP3.
4. Was rotation variance is created randomly?: Yes it was
TODO: explain more details about rotation experiment, 



"When the the rotation variance is created for the testing dataset, was this random? Also, what would happen if the rotation was in x-axis or y-axis or both x- and y- axes or all axes? How is the performance affected if those rotations happen?"
TODO: explain more detailed about rotation experiment, 

#Draft version

We thank the reviewers for their feedback. We are glad to receive positive comments that value the contribution of our work. In summary, we group reviewer concern into three main problems.

The first one is the effectiveness of our architecture. Reviewer 3 ask why we do not provide any results for 3D SegCaps for other datasets beside iSeg2017 and the reason it's we can only train 3D SegCaps successfully if we set the training batch size to 1 or it will produce very low result which have been shown in [24]. Because of this plus high computational cost of capsule network due to iterative routing algorithm, we only train 3D SegCaps for the smallest dataset iSeg2017 which has 9 samples. On the other hand, our network with convolutional decoder do not suffer from this problem and for example, we can train with batch size 32 for patch size (32, 32, 32) on 32GB V100 GPU. Our hypothesis for this empirical finding, which also address reviewer 1 concern on our expanding path, is routing algorithm working based on routing-by-agreement between part to whole relationship, however the relationship between whole to part is one-to-many, we do not find the agreement between whole to active corresponding parts. Then we think the job of expanding path is learning the latent representation of the "whole" capsules from contracting path and replicating the knowledge spatially, which is the purpose of convolutational layers
#####Then we think the job of expanding path is learning the latent representation of the "whole" capsules from contracting path and replicating the knowledge spatially, which is the purpose of convolutational layers

The second one is the experimental choices in our work. Our motivation for robustness experiment come from the reporting of iSeg2017 challenge [26] in which all methods consistently performed badly on the testing subjects acquired with motion artifacts and unusual scan pose. Among participant methods, 3D SkipDense not only stand out because of its performance but they also publish their code and pretrained model on github. Then we can easily check the result and perform our robustness experiment on their model. About the rotation invariance experiment, the result was collected by rotating the testing subject around z-axis with different angles in this order: 0, 5, 15, 30, 45, 60, 75, 90 then there was no random as reviewer 3 concerned. The same results was collected if we rotate testing subject around x-axis, y-axis or all axis as reviewer 3 suggested but we did not have enough space to put these results into the paper. Then we will show them below

| Rotate axis | Model           | 0     | 5     | 15    | 30    | 45    | 60    | 75    | 90    |
|-------------|-----------------|-------|-------|-------|-------|-------|-------|-------|-------|
| x           | 3D-SkipDense    | 92.51 | 89.86 | 72.98 | 74.25 | 86.70 | 85.64 | 84.89 | 85.96 |
|             | 3D-UCaps (ours) | 92.17 | 89.53 | 89.09 | 87.92 | 86.70 | 85.64 | 84.89 | 85.96 |
| y           | 3D-SkipDense    | 92.51 | 89.36 | 69.51 | 76.06 | 74.25 | 74.25 | 74.25 | 74.25 |
|             | 3D-UCaps (ours) | 92.17 | 89.41 | 89.01 | 88.22 | 87.46 | 86.86 | 86.47 | 88.01 |
| all         | 3D-SkipDense    | 92.51 | 89.67 | 82.97 | 83.02 | 74.25 | 74.25 | 74.25 | 74.25 |
|             | 3D-UCaps (ours) | 92.17 | 89.67 | 82.97 | 83.02 | 74.25 | 74.25 | 74.25 | 74.25 |

The last one is the reproducibility and expandability of our work. We have refactored our code so it use MONAI framework for processing data, running sliding window inference and computing dice score with fixed seed. We also follow Pytorch Lightning framework to organize our code effectively. We hope that by using these popular and up-to-date frameworks, anyone in the community can reproduce our results correctly and extend our method easily to other problems as reviewer 1 suggested.

%TODO: explain more detailed about rotation experiment, 
%The result was collected by rotating the testing subject around z-axis with different angles in this order: 0, 5, 15, 30, 45, 60, 75, 90 then there was no random here. The same results was collected if we rotate testing subject around x-axis, y-axis or all axis as you can see in the table below

%| Rotate axis | Model           | 0     | 5     | 15    | 30    | 45    | 60    | 75    | 90    |
%|-------------|-----------------|-------|-------|-------|-------|-------|-------|-------|-------|
%| x           | 3D-SkipDense    | 92.51 | 89.38 | 88.99 | 88.16 | 87.16 | 86.27 | 85.59 |  |
%|             | 3D-UCaps (ours) | 92.17 | 89.53 | 89.09 | 87.92 | 86.70 | 85.64 | 84.89 | 85.96 |
%| y           | 3D-SkipDense    | 92.51 | 89.46 | 89.17 | 88.67 | 88.06 | 87.53 | 87.10 | 89.13 |
%|             | 3D-UCaps (ours) | 92.17 | 89.41 | 89.01 | 88.22 | 87.46 | 86.86 | 86.47 | 88.01 |
%| all         | 3D-SkipDense    | 92.51 | 87.70 | 86.90 | 85.33 | 83.84 | 83.00 | 82.47 | 85.28 |
%|             | 3D-UCaps (ours) | 92.17 | 88.17 | 87.26 | 85.09 | 83.40 | 82.05 | 81.12 | 83.64 |

| Rotate axis | Model           | 0     | 5     | 15    | 30    | 45    | 60    | 75    | 90    |
|-------------|-----------------|-------|-------|-------|-------|-------|-------|-------|-------|
| x           | 3D-SkipDense    | 92.60 | 89.38 | 88.99 | 88.16 | 87.16 | 86.27 | 85.59 | 87.04 |
|             | 3D-UNet         | 92.48 | 89.61 | 89.16 | 87.98 | 86.74 | 85.63 | 84.97 | 86.41 |
|             | 3D-UCaps (ours) | 92.54 | 89.79 | 89.23 | 88.00 | 86.71 | 85.65 | 84.97 | 86.31 |
| y           | 3D-SkipDense    | 92.60 | 89.46 | 89.17 | 88.67 | 88.06 | 87.53 | 87.10 | 89.13 |
|             | 3D-UNet         | 92.48 | 89.61 | 89.16 | 88.21 | 87.30 | 86.69 | 86.19 | 87.87 |
|             | 3D-UCaps (ours) | 92.54 | 89.82 | 89.40 | 88.53 | 87.79 | 87.19 | 86.73 | 88.49 |
| all         | 3D-SkipDense    | 92.60 | 87.70 | 86.90 | 85.33 | 83.84 | 83.00 | 82.47 | 85.28 |
|             | 3D-UNet         | 92.48 | 88.29 | 87.14 | 84.94 | 83.22 | 82.06 | 81.13 | 83.81 |
|             | 3D-UCaps (ours) | 92.54 | 88.46 | 87.27 | 85.13 | 83.58 | 82.48 | 81.64 | 84.27 |

==> submission/tmp/rebuttal_Tan.tex <==
#Draft version

We thank the reviewers for their feedback. We are glad to receive positive comments that value the contribution of our work. In summary, we group reviewer concern into three main problems.

The first one is the effectiveness of our architecture. Reviewer 3 ask why we do not provide any results for 3D SegCaps for other datasets beside iSeg2017 and the reason it's we can only train 3D SegCaps successfully if we set the training batch size to 1 or it will produce very low result which have been shown in [24]. Because of this plus high computational cost of capsule network due to iterative routing algorithm, we only train 3D SegCaps for the smallest dataset iSeg2017 which has 9 samples. On the other hand, our network with convolutional decoder do not suffer from this problem and for example, we can train with batch size 32 for patch size (32, 32, 32) on 32GB V100 GPU. Our hypothesis for this empirical finding, which also address reviewer 1 concern on our expanding path, is routing algorithm working based on routing-by-agreement between part to whole relationship, however the relationship between whole to part is one-to-many, we do not find the agreement between whole to active corresponding parts. Then we think the job of expanding path is learning the latent representation of the "whole" capsules from contracting path and replicating the knowledge spatially, which is the purpose of convolutational layers

The second one is the experimental choices in our work. Our motivation for robustness experiment come from the reporting of iSeg2017 challenge [26] in which all methods consistently performed badly on the testing subjects acquired with motion artifacts and unusual scan pose. Among participant methods, 3D SkipDense not only stand out because of its performance but they also publish their code and pretrained model on github. Then we can easily check the result and perform our robustness experiment on their model. About the rotation invariance experiment, the result was collected by rotating the testing subject around z-axis with different angles in this order: 0, 5, 15, 30, 45, 60, 75, 90 then there was no random as reviewer 3 concerned. The same results was collected if we rotate testing subject around x-axis, y-axis or all axis as reviewer 3 suggested but we did not have enough space to put these results into the paper. Then we will show them below

| Rotate axis | Model           | 0     | 5     | 15    | 30    | 45    | 60    | 75    | 90    |
|-------------|-----------------|-------|-------|-------|-------|-------|-------|-------|-------|
| x           | 3D-SkipDense    | 92.51 | 89.86 | 72.98 | 74.25 | 86.70 | 85.64 | 84.89 | 85.96 |
|             | 3D-UCaps (ours) | 92.17 | 89.53 | 89.09 | 87.92 | 86.70 | 85.64 | 84.89 | 85.96 |
| y           | 3D-SkipDense    | 92.51 | 89.36 | 69.51 | 76.06 | 74.25 | 74.25 | 74.25 | 74.25 |
|             | 3D-UCaps (ours) | 92.17 | 89.41 | 89.01 | 88.22 | 87.46 | 86.86 | 86.47 | 88.01 |
| all         | 3D-SkipDense    | 92.51 | 87.70 | 86.90 | 85.33 | 83.84 | 83.00 | 82.47 | 85.28 |
|             | 3D-UCaps (ours) | 92.17 | 88.17 | 87.26 | 85.09 | 83.40 | 82.05 | 81.12 | 83.64 |

The last one is the reproducibility and expandability of our work. We have refactored our code so it use MONAI framework for processing data, running sliding window inference and computing dice score with fixed seed. We also follow Pytorch Lightning framework to organize our code effectively. We hope that by using these popular and up-to-date frameworks, anyone in the community can reproduce our results correctly and extend our method easily to other problems as reviewer 1 suggested. 
